GaussianRoom: Improving 3D Gaussian Splatting with SDF Guidance and Monocular Cues for Indoor Scene Reconstruction

Embodied intelligence requires precise reconstruction and rendering to simulate large-scale real-world data. Although 3D Gaussian Splatting (3DGS) has recently demonstrated high-quality results with real-time performance, it still faces challenges in indoor scenes with large, textureless regions, resulting in incomplete and noisy reconstructions due to poor point cloud initialization and underconstrained optimization. Inspired by the continuity of signed distance field (SDF), which naturally has advantages in modeling surfaces, we propose a unified optimization framework that integrates neural signed distance fields (SDFs) with 3DGS for accurate geometry reconstruction and real-time rendering. This framework incorporates a neural SDF field to guide the densification and pruning of Gaussians, enabling Gaussians to model scenes accurately even with poor initialized point clouds. Simultaneously, the geometry represented by Gaussians improves the efficiency of the SDF field by piloting its point sampling. Additionally, we introduce two regularization terms based on normal and edge priors to resolve geometric ambiguities in textureless areas and enhance detail accuracy. Extensive experiments in ScanNet and ScanNet++ show that our method achieves state-of-the-art performance in both surface reconstruction and novel view synthesis.

==> table_tex.tex <==
\begin{table*}[!h]
    \centering
    % \renewcommand\arraystretch{0.95}
    \scalebox{0.97}
    {
    \begin{tabular}{l|cccc>{\columncolor[gray]{0.902}}c}
    \hline
    Method      & Accuracy$\downarrow$     & Completion$\downarrow$   & Precision$\uparrow$    & Recall$\uparrow$       & \textbf{F-score}$\uparrow$      \\ \hline
    COLMAP \cite{schonberger2016structure}      & 0.062 / 0.091 & 0.090 / 0.093 & 0.640 / 0.519 & 0.569 / 0.520 & 0.600 / 0.517 \\ \hline
    NeRF \cite{mildenhall2021nerf}        & 0.160 / 0.135 & 0.065 / 0.082 & 0.378 / 0.421 & 0.576 / 0.569 & 0.454 / 0.484 \\
    NeuS \cite{wang2021neus}        & 0.105 / 0.163 & 0.124 / 0.196 & 0.448 / 0.316 & 0.378 / 0.265 & 0.409 / 0.288 \\
    MonoSDF \cite{yu2022monosdf}     & 0.048 / 0.039 & 0.068 / 0.043 & 0.673 / 0.816 & 0.558 / 0.840 & 0.609 / 0.827 \\
    HelixSurf \cite{liang2023helixsurf}   & 0.063 / \ \ \ \ -  \ \ \ \  & 0.134 / \ \ \ \ -  \ \ \ \     & 0.657 / \ \ \ \ -  \ \ \ \     & 0.504 / \ \ \ \ -  \ \ \ \     & 0.567 / \ \ \ \ -  \ \ \ \     \\ \hline
    3DGS \cite{kerbl20233dgs} & 0.338 / 0.113 & 0.406 / 0.790 & 0.129 / 0.445 & 0.067 / 0.103 & 0.085 / 0.163 \\
    GaussianPro \cite{cheng2024gaussianpro} & 0.313 / 0.141 & 0.394 / 1.283 & 0.112 / 0.353 & 0.075 / 0.081 & 0.088 / 0.129 \\
    SuGaR \cite{guedon2023sugar}       & 0.167 / 0.129 & 0.148 / 0.121 & 0.361 / 0.435 & 0.373 / 0.444 & 0.366 / 0.439 \\ 
    DN-Splatter \cite{turkulainen2024dn} & 0.212 / 0.294 & 0.210 / 0.276 & 0.153 /0.108  & 0.182 / 0.108 & 0.166 / 0.107 \\ \hline
    Ours        & \textbf{0.047} / \textbf{0.035} & \textbf{0.043} / \textbf{0.037} & \textbf{0.800} / \textbf{0.894} & \textbf{0.739} / \textbf{0.852} & \textbf{0.768} / \textbf{0.872} \\ \hline
    \end{tabular}
    }
    \caption{\textbf{Quantitative reconstruction comparison} on ScanNet / ScanNet++ datasets. We report the average results over 8 and 2 scenes respectively. The best results are marked in \textbf{bold}.}
    \label{tab:table1}
    \vspace{-0.3cm}
\end{table*}
